Practical Privacy Filters and Odometers with R\'enyi Differential Privacy and Applications to Differentially Private Deep Learning

Differential Privacy (DP) is the leading approach to privacy preserving deep learning. As such, there are multiple efforts to provide drop-in integration of DP into popular frameworks. These efforts, which add noise to each gradient computation to make it DP, rely on composition theorems to bound the total privacy loss incurred over this sequence of DP computations. However, existing composition theorems present a tension between efficiency and flexibility. Most theorems require all computations in the sequence to have a predefined DP parameter, called the privacy budget. This prevents the design of training algorithms that adapt the privacy budget on the fly, or that terminate early to reduce the total privacy loss. Alternatively, the few existing composition results for adaptive privacy budgets provide complex bounds on the privacy loss, with constants too large to be practical. In this paper, we study DP composition under adaptive privacy budgets through the lens of R\'enyi Differential Privacy, proving a simpler composition theorem with smaller constants, making it practical enough to use in algorithm design. We demonstrate two applications of this theorem for DP deep learning: adapting the noise or batch size online to improve a model's accuracy within a fixed total privacy loss, and stopping early when fine-tuning a model to reduce total privacy loss.

==> Makefile <==
PAPER=paper
LATEX=pdflatex

BIBTEX=bibtex

SRCS=$(PAPER).tex $(wildcard sections/*.tex)
REFS=$(wildcard bib/*.bib)
FIGS=$(wildcard figures/*)
STYLE=$(wildcard style/*)

.PHONY: results $(PAPER).pdf clean

all: $(PAPER).pdf

results:
	+make -C $@

$(PAPER).pdf: $(SRCS) $(REFS) $(FIGS) $(STYLE)
	$(LATEX) $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX) $(PAPER)
	$(LATEX) $(PAPER)


submission: $(PAPER).pdf
	cp $(PAPER).pdf submission/

clean:
	rm -f *.out *.dvi *.aux *.log *.blg *.bbl \
          $(PAPER).ps $(PAPER).pdf \
          $(PAPER)-single.pdf $(PAPER)-single.ps


==> sections/early-stopping.tex <==
\section{Early Stopping}

Our privacy filter enables users to adaptively chose the RDP budget of each query, and ensures that a global budget is not overreached.
However, it does not let a user know how much budget has been spent so far, and stop querying at any moment with only this budget spent.
This is the goal of a privacy odometer.
To construct such an odometer for RDP that also translates to strong DP guarantees, we first study a more restricted adaptive setup: early stopping
In this setup, the RDP budget used by each query is either a number fixed in advance, or zero until the end. That is, the sequence of budgets is fixed in advance, but one can decide to stop querying at anytime to strop spending budget. This stopping can depend on past outcomes, and in this sense, the budget is adaptive.

Interestingly, \cite{10.5555/3157096.3157312} proves a lower bound for privacy accounting even in this restrictive adaptive setup.
Their Theorem 6.1 shows that for a sequence of $\epsilon$-DP ($(\infty, \epsilon)$-RDP)  queries with adaptive stopping, the budget consumed when stopping after $n$ queries is at least $\cO(\epsilon\sqrt{n \log(\frac{\log(k)}{\delta})})$ ---instead of $\cO(\epsilon\sqrt{n \log(\frac{1}{\delta})})$---, where $k$ is the maximum number of queries that could be performed.

\subsection{Setup}
We use the following interaction setup for composition:

\begin{algorithm}[H]
  \caption{$\textrm{EarlyStoppingComp}(A,k,b, \alpha, \epsilon=(\epsilon_1, \ldots, \epsilon_k))$}
  \label{early-stopping-comp}
\begin{algorithmic}
  \FOR {$i = 1, \ldots, k$}
    \STATE $A = A(v_1, \ldots, v_{i-1})$\;
    \STATE $A$ gives neighboring $D_i^{0}, D_i^{1}, \epsilon_i, \textrm{and~} M_i: \cD \rightarrow \cR$ an $(\alpha, \epsilon_i)$-RDP mechanism\;
    \STATE $A$ receives $v_i \sim V^b_i = M_i(D_i^{b})$\;
    \STATE $A = A(v_1, \ldots, v_{i})$ decides to \{CONTINUE, STOP\}\;
    \IF {$A$ STOPs}
      \STATE BREAK\;
    \ENDIF
    \ENDFOR
  \OUTPUT stopping time $s=i$ and view $V^b=(v_1, \ldots, v_s)$.
\end{algorithmic}
\end{algorithm}

\subsection{RDP Analysis}

In words, the adversary interacts with the data through a sequence of $(\alpha, \epsilon_i)$-RDP mechanisms. The $\epsilon_i$ are fixed in advance (passed as parameters), but the adversary can stop the interaction at any time.
%
To define an RDP guarantee for Algorithm \ref{early-stopping-comp}, we introduce a conditional version of the R\'enyi Divergence:
\[
  D_\alpha(P || Q \big| s) \triangleq \frac{1}{\alpha - 1} \log \E_{x \sim Q} \big[\Big( \frac{P(x)}{Q(x)} \Big)^\alpha \big| s \big] .
\]

Here we condition on the stopping time, but we can condition on other events as well. Given this definition, we are ready to state an RDP guarantee for early stopping. While this result is rather straight forward, it will be crucial to study DP implications in the next subsection (\S\ref{sec:dp-early-stopping}) and odometers (\S\ref{sec:odometers}).

\begin{theorem}[RDP Early-Stopping]
\label{prop:rdp-early-stopping}
The interaction mechanism from Algorithm \ref{early-stopping-comp} is such that:
\[
  \forall s \in [1, k] \negmedspace : D_\alpha(V^0_{\leq k} || V^1_{\leq k} \big| s) \leq \sum_{i=1}^s \epsilon_i .
\]
\end{theorem}
\begin{proof}
$D_\alpha(V^0_{\leq k} || V^1_{\leq k} \big| s) = D_\alpha(V^0_{\leq s} || V^1_{\leq s}) \leq \sum_{i=1}^s \epsilon_i$ where the inequality is the usual RDP composition theorem since the $\epsilon_i$ are fixed in advance.
\end{proof}

\subsection{Differentially Private Early Stopping}
\label{sec:dp-early-stopping}

We cannot translate this RDP result to an $(\epsilon, \delta)$-DP guarantee as-is however, because of the adaptive stopping.
Remember from \S\ref{sec:privacy-background} that 

The most straight forward way to do this is to apply a union bound over all $l$ possible stopping times. Directly applying this to the whole R\'enyi curve composition (similarly to \S\ref{sec:filter-renyi-curve}, where $\epsilon_i$ becomes $\epsilon_i(\alpha)$) yields that the early stopping mechanism is: $\Big(\sum \epsilon_i(\alpha) + \frac{\log(l/\delta)}{\alpha - 1}, \delta\Big)\textrm{-DP}$.
However in most cases we will want to avoid a direct dependency on $l$. This is because $l$ may not be known in advance, and it is more practical to set it extremely large so it is not a limitation. We thus treat t
\begin{theorem}[DP Early-Stopping]
\label{prop:early-stopping}
  The interaction mechanism from Algorithm \ref{early-stopping-comp}, is such that with probability at least $1-\delta$, for all $s \in [1, k]$ we have: $\big| \log\big(\frac{P(V^0_{\leq s})}{P(V^1_{\leq s})}\big) \big| \leq \sum_{i=1}^s \epsilon_i(\alpha) + \frac{\log(2s^2/\delta)}{\alpha - 1}$.
\end{theorem}
\begin{proof}
As in Theorem \ref{prop:rdp-early-stopping}, $\forall s \negmedspace : D_\alpha(V^0_{\leq s} || V^1_{\leq s}) \leq \sum_{i=1}^s \epsilon_i$, which in turn implies from Eq. \ref{rdp-to-dp} that with probably at least $1-\beta_s$, $|\log\big(\frac{P(V^0_{\leq s})}{P(V^1_{\leq s})}\big)| \leq \sum_{i=1}^s \epsilon_i(\alpha) + \frac{\log(1/\beta_s)}{\alpha - 1}$.

  We choose $\beta_s = \frac{\delta}{2s^2}$. Since $\sum_{i=1}^k \beta_i < \delta$, applying a union bound concludes the proof.
\end{proof}

Theorem \ref{prop:early-stopping} means that with probability at least $1-\delta$ over the whole interaction, $\sum \epsilon_i(\alpha) + \frac{\log(l/\delta)}{\alpha - 1}$ is a running upper-bound on the privacy loss of the outcome of Algorithm \ref{early-stopping-comp}.
This is the definition of a privacy odometer from \cite{10.5555/3157096.3157312}.
Theorem \ref{prop:early-stopping} also applies for all $\alpha$ where  $\epsilon_i$ becomes $\epsilon_i(\alpha)$, yielding a strong DP composition through RDP.
So far however, our privacy odometer is limited to early stopping with fixed $\epsilon_i(\alpha)$ parameters.


